Some Reflections on Drawing Causal Inference using Textual Data: Parallels Between Human Subjects and Organized Texts

We examine the role of textual data as study units when conducting causal inference by drawing parallels between human subjects and organized texts. %in human population research. We elaborate on key causal concepts and principles, and expose some ambiguity and sometimes fallacies. To facilitate better framing a causal query, we discuss two strategies: (i) shifting from immutable traits to perceptions of them, and (ii) shifting from some abstract concept/property to its constituent parts, i.e., adopting a constructivist perspective of an abstract concept. We hope this article would raise the awareness of the importance of articulating and clarifying fundamental concepts before delving into developing methodologies when drawing causal inference using textual data.

==> include/macros.tex <==
%!TEX root = ../main.tex


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\DeclareMathOperator*{\argmin}{arg\,min}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{remark}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{assumption}{Assumption}
\newtheorem*{assumption*}{Assumption}
\newtheorem{side_info}{Side-Information}
% \newtheorem{proposition}{Proposition}
% \newtheorem{condition}{Condition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{constraint}{Constraint}


\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\makeatletter
\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
\renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
\def\@algocf@capt@plain{top}
\renewcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
  \hskip .5\algomargin%
  \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
  \global\@minipagefalse%
  \hbox to\hsize{\box\@tempboxa}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}
\makeatother


==> include/packages.tex <==
%!TEX root = ../main.tex
\usepackage[utf8]{inputenc}
\usepackage{bm, bbm,commath}
\usepackage{natbib}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amssymb}
\usepackage{blkarray}
\usepackage{multicol}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{textcomp}

\usepackage{sectsty}
\setcounter{MaxMatrixCols}{30}
% \usepackage[onehalfspacing]{setspace}

% \linespread{1.5}

% \usepackage[usenames,dvipsnames]{color}
% \usepackage{float}


==> nkgfsskgmdxdxjnrjztqfmthbbdhcgdk/abstract.tex <==
\begin{abstract}%
    We examine the role of textual data as \emph{study units}
    when conducting causal inference by drawing parallels between human subjects and organized texts. %in human population research.
    We elaborate on key causal concepts and principles, and expose some ambiguity and sometimes fallacies. To facilitate better framing a causal query, we discuss two strategies: (i) shifting from immutable traits to perceptions of them, and (ii) shifting from some abstract concept/property to its constituent parts, i.e., adopting a constructivist perspective of an abstract concept. We hope this article would raise the awareness of
    the importance of articulating and clarifying fundamental concepts before delving into developing methodologies when drawing causal inference using textual data.
\iffalse
\jiayao{Interesting version}
In a 1900 Royal Institution lecture, William Thomson, the first Baron Kelvin of Largs in the County of Ayr, vividly
described that
``\emph{the beauty and clearness of the dynamical theory is at present obscured by two clouds. The first came into existence with the undulatory theory of light, the second is the Maxwell–Boltzmann doctrine regarding the partition of energy.}''
In a similar vein, the same can be said for the \emph{status quo}
of applying causal inference to natural languages:
the first cloud being the confusion of immutable traits; and the
second oblivion to account for all mutable traits.
In this article, we attempt to clear out these clouds by
paralleling organized texts as study units with human subjects,
where time-honored wisdoms have been formed through
trials-and-errors, pitfalls and progresses.
We discuss principles and caveats of framing
    proper causal queries, and articulate possible mitigation strategies, namely, (i) a shift from immutable traits to perceptions;
    (ii) a constructivism from perceptions to a bundle of states.
We hope this article would raise the awareness of
    the importance of clarifying fundamental questions
    of drawing causal conclusions based on textual data
    that becomes more quintessential in the natural
    language processing literature, and eventually
    leads to solid foundations that are comparable
    to special and general relativity did to modern physics.
\fi    
\end{abstract}
\begin{keywords}%
Causal inference; Constructivism; Natural language processing; Potential outcomes framework; Pretreatment variables
\end{keywords}

==> nkgfsskgmdxdxjnrjztqfmthbbdhcgdk/include/macros.tex <==
%!TEX root = ../main.tex


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\DeclareMathOperator*{\argmin}{arg\,min}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{remark}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{assumption}{Assumption}
\newtheorem*{assumption*}{Assumption}
\newtheorem{side_info}{Side-Information}
% \newtheorem{proposition}{Proposition}
% \newtheorem{condition}{Condition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{constraint}{Constraint}


\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\makeatletter
\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
\renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
\def\@algocf@capt@plain{top}
\renewcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
  \hskip .5\algomargin%
  \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
  \global\@minipagefalse%
  \hbox to\hsize{\box\@tempboxa}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}
\makeatother


==> nkgfsskgmdxdxjnrjztqfmthbbdhcgdk/include/packages.tex <==
%!TEX root = ../main.tex
\usepackage[utf8]{inputenc}
\usepackage{bm, bbm,commath}
\usepackage{natbib}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amssymb}
\usepackage{blkarray}
\usepackage{multicol}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{textcomp}

\usepackage{sectsty}
\setcounter{MaxMatrixCols}{30}
% \usepackage[onehalfspacing]{setspace}

% \linespread{1.5}

% \usepackage[usenames,dvipsnames]{color}
% \usepackage{float}

